Entropy of real rational surface automorphisms: Actions on the Fundamental Groups

This article discusses a method to compute the induced action on the fundamental group of a real rational surface and provides the induced actions for basic quadratic real automorphisms. Using an invariant set in the fundamental group, we introduce a method to estimate a lower bound of the action's growth rate on the fundamental group. The growth rate of this induced action gives a lower bound for the entropy of real surface automorphism.

==> GRateV2.tex <==
Let $f_\mathbf{R}$ be the real diffeomorphism with the determinant $>1$ associated with the orbit data $n_1, n_2, n_3$ and a cyclic permutation.  For the rest of this article, let us fix a set of generators for $\pi_1(X(\mathbf{R}, P_{fix}))$, \[G = \{ e, a_i, b_j, c_k, 1 \le i \le  n_3, 1 \le j \le n_1, 1 \le k \le n_2\}\] as defined in the Section \ref{S:Action}. Let $G^{-1} = \{ g^{-1} : g \in G\}$ denote the set of inverses of generators in $G$. 
Let $\ell_G (\omega)$ denote the minimal word length of an element $\omega \in \pi_1(X(\mathbf{R}), P_{fix})$ with respect to the set of generators $G$. The growth rate of the induced action $f^{-1}_{\mathbf{R}*}: \pi_1(X(\mathbf{R}), P_{fix}) \to \pi_1(X(\mathbf{R}), P_{fix})$ is defined by 
\[ \rho (f^{-1}_{\mathbf{R}*}) := \sup_{g \in G} \left \{ \  \limsup_{n \to \infty} \, (\ell_G ( f^{-n}_{\mathbf{R}*} g))^{1/n}\  \right \}. \]
The growth rate of the induced action on the fundamental group gives the lower estimate for the topological entropy.
\begin{thm}\cite{Bowen}
Let $f:M \to M$ be a map of a compact manifold and let $\mu$ be the growth rate of the induced action $f_*$ on $\pi_1(M)$. Then \[ h_{top}(f) \ge log \mu \]
\end{thm}

Since the fundamental group of $X(\mathbf{R})$ is non-commutative with one relator, it is hard to compute the growth rate. To overcome the difficulties, we use the conjugacy classes of the fundamental group, in other words, the base free homotopy classes. For each $\omega \in \pi_1(X(\mathbf{R}), P_{fix})$, let $\ell (\omega)$ denote the minimal word length in the conjugacy class $[\omega]$
\[ \ell (\omega) = \min \{ \ell_G (x) : x = y \omega y^{-1}, y \in \pi_1(X(\mathbf{R}), P_{fix}) \}. \] 
We say a word $w=g_{i_1} \cc g_{i_2} \cc \cdots \cc g_{i_n}$, $g_{i_j} \in G \cup G^{-1}$ for $j=1, \dots n$ is \textit{G-cyclically reduced} if every cyclic permutation of $w$ is written in the shortest length using the relations in $G$, in other words (1) $g_{i_j} g_{i_{j+1}} \ne 1$ for all $j = 1, \dots n$ modulo $n$ and (2) each cyclic permutation of $w$ is reduced using the unique relators in generators in $G$ and thus it is written in a word with shortest length. It is clear that $\ell (\omega) \le \ell_G(\omega)$ and the equality holds if $\omega$ is $G$-cyclically reduced. The following Lemma is useful for us. 
\begin{lem}\label{L:cpconj}
If two $G$-cyclically reduced words are in the same conjugacy class, one is a cyclic permutation of another. 
\end{lem}
\begin{proof}
If $\omega \in \pi_1(X(\mathbf{R}), P_{fix})$ is a $G$-cyclically reduced with respect to a set of generator $G$, then $\omega = g_{i_1} \cdots g_{i_n}$ where $g_{i_1} \ne g_{i_n}^{-1}$ and $\ell_G(\omega)= n$. Thus for any  $g \in G \cup G^{-1} $, $\ell_G( g \omega g^{-1}) \ge \ell_G(\omega)$ and the equality holds only if $g = g_{i_1}^{-1}$ or $g= g_{i_n}$. Also for any reduced word $x \in \fun$, $\ell_G( x \omega x^{-1}) \ge \ell_G(\omega)$ and equality holds only if there is an index $1\le j\le n$ such that either $x^{-1} =   g_{i_1} \cdots g_{i_j}$ or $x =  g_{i_j} \cdots g_{i_n}$. It follows that for a $G$-cyclically reduced word $\omega$, $\ell(\omega) = \ell_G(\omega)$ and if $\omega'$ is a conjugation of $\omega$ with the property that $\ell_G(\omega) = \ell_G(\omega')$ then $\omega'$ is a cyclic permutation of $\omega$.
Since two $G$-cyclically reduced words in$\omega_1$ and $\omega_2$  the same conjugacy class satisfy $\ell(\omega_1)=\ell_G(\omega_1) = \ell_G(\omega_2)=\ell(\omega_2)$, we see that $\omega_1$ is a cyclic permutation of $\omega_2$.
\end{proof}
In \cite{Birman-Series}, Birman and Series considered an automorphism $\phi$ on the fundamental group of a compact surface $M$ and showed there is a family of cyclic words $W$ with respect to a set of generators of $\pi_1(M)$ such that an appropriate restriction of $\phi$ on the positive span of $W$ is linear. To use Whitehead's idea in \cite{whitehead}, Birman and Series construct $W$ such that a group generated by $W$ is free and study the induced map on the positive span $Sp^+(W)$ to show its linearity and the growth rate. To estimate the growth rate of the induced action on the fundamental group, we adapt the idea of Birman and Series \cite{Birman-Series}.

\subsection{Invariant Set of admissible sequences}\label{SS:admissible} Let $\Gamma=\{ \gamma_1, \dots, \gamma_k\}$ be a finite set of distinct reduced words in $\pi_1(X(\mathbf{R}), P_{fix})$ with respect to a set of generator $G$ with the following properties: For each  $\gamma = g_1 \cdots g_s \in \Gamma$,
\begin{itemize}
\item the length $\ell_G(\gamma) = \ell (\gamma) = s \ge 2$,
\item there is $g$ in a symmetric set $ G\cup G^{-1} = \{ g, g^{-1}: g\in G\}$, such that $g_s=g$, $g_{j} \ne g $ for all $1 \le j \le s-1$, and
\item $\gamma$ is a $G$-cyclically reduced word in $\pi_1(X(\mathbf{R}), P_{fix})$, i.e. $g_1 \ne g^{-1}$. 
\end{itemize}

Let $\Gamma^+$ be a monoid of words in $\Gamma$ such that each $\gamma \in \Gamma^+$ is written as a product of positive powers of $\gamma_i$'s:
\[ \Gamma^+ = \{ \gamma = \gamma_{i_1}^{\epsilon_1} \cc \dots \gamma_{i_s}^{\epsilon_s}: \gamma_{i_j} \in \Gamma, \text{  and } s, \epsilon_1, \dots \epsilon_s \ge 0\}. \]
For each $\gamma \in \ \Gamma ^+$, let $\ell_\Gamma (\gamma)$ denote the minimal word length in $\Gamma$. Since the unique relator for the set of generator $G$ for the fundamental group of $X(\mathbf{R})$ is given by the product of squares of generators and each $\gamma\in \Gamma^+$ is given by a product of positive powers of $\gamma_i\in \Gamma$ , there is no relation in $\Gamma^+$.  It follows that 


\begin{lem}\label{L:Gplus} Every word in $\Gamma ^+$ is $G$-cyclically reduced with respect to a set of generators $G$. Thus for each $\gamma= \gamma_{i_1}\gamma_{i_2} \dots \gamma_{i_n} \in  \Gamma ^+$ \[ \ell (\gamma)=\ell_G (\gamma)  = \sum_{j=1}^n \ell (\gamma_{i_j})  \quad \text{and} \quad \ell_\Gamma (\gamma)= \sum_{ i =1}^k n_i(\gamma)\] where $n_i (\gamma)$ is the number of $\gamma_i$ in the word $\gamma$.
\end{lem}

\begin{proof}
Every $\gamma_i \in \Gamma$ starts with a letter $\ne g, g^{-1}$ and ends with a letter $g$ or $g^{-1}$. Since the unique relation on a set of generators $G$ is given by a product of squares of elements in $G$, any length reduction, if there are any, must happen in each $\gamma_i$. Each $\gamma_i \in \Gamma$ is a reduced word with respect to $G$. Thus any word in $\gamma \in \Gamma^+$ is reduced with respect to $G$ and the length $\ell(\gamma) = \ell_G(\gamma)$ depends only on the number of $\gamma_i's$ in $\Gamma$.
\end{proof}

Let  $\langle \Gamma^+ \rangle := \{ [\gamma] : \gamma \in \Gamma^+\}$ be a set of conjugacy classes of $\Gamma^+$ in $\pi_1(X(\mathbf{R}), P_{fix})$. Using Lemma \ref{L:cpconj} and Lemma \ref{L:Gplus}, we have that  for $\gamma, \gamma' \in \Gamma^+$, $\gamma$ and $\gamma'$ are cyclic permutation with respect to $\gamma_i$'s in $\Gamma$ if and only if the $[\gamma] = [\gamma']$. Also we see that the length $\ell_\Gamma$ is well defined in $\langle \Gamma^+ \rangle$, that is for each $[\gamma] \in \langle \Gamma^+ \rangle$ we have
\[ \ell_\Gamma [\gamma] = \ell_\Gamma (\gamma). \]

\subsubsection{Admissible sequences}\label{SS:admissible}
Let $A$ be a set of ordered $n$-tuples in $\{1, 2, \dots, k\}$. We say a word $\gamma= \gamma_{i_1} \cdots \gamma_{i_n}\in \Gamma^+$ of length $n$ is \textit{an $A$-admissible $n$ block} if the $n$-tuple of indices $(i_1, \dots, i_n) \in A$. We say a finite word $\gamma$ in $\Gamma^+$ is \textit{cyclically admissible with respect to $A$}, (or simply \textit{$A$-admissible}) if each $n$ blocks in $\gamma$  is an $A$-admissible $n$ block. Let $\Gamma_A \subset \langle \Gamma^+ \rangle$ be a set of conjugacy classes of (cyclically) $A$-admissible cyclic words in $\Gamma^+$.
\[ \Gamma_A = \{ [\gamma] \in \langle \Gamma^+ \rangle: \gamma= \gamma_{i_1} \cdots \gamma_{i_s}, s\ge n, (i_j, \dots i_{j+n}) \in A \} \]
where the indexes are taken modulo $s = \ell_\Gamma (\gamma)$.


When $[f^{-1}_{\mathbf{R}*} \gamma] \in \Gamma_A$ for every $[\gamma] \in \Gamma_A$, i.e. there is $\gamma' \in \Gamma_A$ such that   $f^{-1}_{\mathbf{R}*} \gamma$ is conjugate to $\gamma'$ in $\pi_1(X(\mathbf{R}), P_{fix})$, we say $\Gamma_A$ is $f^{-1}_{\mathbf{R}*}$-invariant. In this case, let us define a map $\phi$ on $\Gamma_A$ by \[ \phi([\gamma]) = [f^{-1}_{\mathbf{R}*} \gamma], \ \ \ \text{for } [\gamma] \in \Gamma_A.\] 
%Since $\Gamma_A$ is a set of cyclic words, $\phi:\Gamma_A \to \Gamma_A$ is well defined. 

%The main focus of this article is estimating the topological entropy. 

For each $[\gamma] \in \Gamma_A$, the length $\ell_\Gamma [\gamma]$ only depends on the number of each $\gamma_i \in \Gamma$ in any representative $\gamma \in [\gamma]$. Let $\text{Sp}^+ \Gamma$ be the positive linear span of $\Gamma$ and for each $[\gamma] \in \Gamma_A$ define $\gamma_\# \in \text{Sp}^+\Gamma$ by 
\begin{equation}\label{E:counting} [\gamma]_\# = \sum_{i=1}^k n_i \gamma_i \quad \text{where  } n_i(\gamma) = \text{the number of } \gamma_i \text{ in } [\gamma].\end{equation}
For instance, if $[\gamma] =[ \gamma_1\gamma_3\gamma_2\gamma_1\gamma_4] \in \Gamma_A$ then $\gamma_\# = 2 \gamma_1 + \gamma_2 +\gamma_3+\gamma_4$. Let $\Gamma_A^\# = \{ \gamma_\#: [\gamma] \in \Gamma_A\}$. 
If $\Gamma_A$ is $f_{\mathbf{R}*}^{-1}$- invariant, for each $[\gamma] \in \Gamma_A$ we have 
\begin{equation} \label{E:cmap}
 (\phi \gamma)_\# \in \Gamma_A^\# 
\end{equation}

\begin{lem}\label{L:linearity} Suppose $\Gamma_A$ is $f_{\mathbf{R}*}^{-1}$-invariant and $ [ \gamma ] ,[\gamma'] \in \Gamma_A$. 
\begin{itemize}
\item For a positive integer $n$, $[\gamma^n]=[  \gamma \gamma \cdots \gamma ]$, the class of the product of $n$ coplies of $\gamma$ is in $\Gamma_A$ and \[ (\phi([\gamma^n]))_\# = n (\phi([\gamma]))_\#\]
\item If two representatives $\gamma$ and $\gamma'$ have the same $n-1$ successive indices then $[\gamma \cc \gamma'] \in \Gamma_A$ and \[ (\phi([\gamma \cc\gamma'])_\# = (\phi([\gamma]))_\# + (\phi([\gamma']))_\#\]
\end{itemize}
\end{lem}

\begin{proof}
Since for $[\gamma], [\gamma'] \in \Gamma_A$,   \[\phi([\gamma\cc  \gamma'] )= [ f^{-1}_{\mathbf{R}*} \gamma \cc \gamma'] =[ f^{-1}_{\mathbf{R}*} \gamma \cc f^{-1}_{\mathbf{R}*}\gamma'],\]
it is enough to show that $[\gamma^n] \in \Gamma_A$ for the first part and $[\gamma\cc \gamma'] \in \Gamma_A$ for the second. 
If $[\gamma]= [\gamma_{i_1} \cdots \gamma_{i_s}] \in \Gamma_A$, every cyclic $n$-sub indices of $\gamma$ is in $A$. Thus it is clear that \[[\gamma^n] = [\gamma_{i_1} \cdots \gamma_{i_s} \gamma_{i_1} \cdots \gamma_{i_s} \dots \gamma_{i_1} \cdots \gamma_{i_s}] \in \Gamma_A. \]
If $\gamma$ and $\gamma'$ have the same $n-1$ successive indices, we may write \[ \gamma = \gamma_{i_1} \cdots \gamma_{i_{n-1}} \cc \gamma_{j_1} \cdots \gamma_{j_s} \quad \text{and} \quad \gamma' = \gamma_{i_1} \cdots \gamma_{i_{n-1}} \cc \gamma_{k_1} \cdots \gamma_{k_t} \]
where $(j_s,i_1, \dots, i_{n-1}), (k_t, i_1 \dots i_{n-1}) \in A$. It follows that 
\[ \gamma\cc \gamma' =  \gamma_{i_1} \cdots \gamma_{i_{n-1}} \cc \gamma_{j_1} \cdots \gamma_{j_s} \cc \gamma_{i_1} \cdots \gamma_{i_{n-1}} \cc \gamma_{k_1} \cdots \gamma_{k_t}\in \Gamma_A\]
\end{proof}

\subsection{Split and Merge}\label{SS:sandp} 
%The set $\Gamma_A$ is not necessarily a semi-group and there is no a priori reason to believe the operation $(\phi [\gamma])_\#$ is linear. To bypass this difficulty we use two linear maps $S$ and $M$  on a linear span of $\Gamma$ . 
%\todo[inline]{define splitting and merging maps}
%
%To estimate the growth rate, we use ``splitting-merging maps".
Let us continue to assume that  $\Gamma_A$ is $f^{-1}_{\mathbf{R}*}$-invariant. Each word $\gamma_i \in \Gamma$ is not necessarily in $\Gamma_A$ and thus a priori $f^{-1}_{\mathbf{R}*} \gamma_i \notin \Gamma^+$. 
However for $[\gamma] = [\gamma_{i_1}\cdots \gamma_{i_n}] \in \Gamma_A$,  we have $\phi[\gamma] = [f^{-1}_{\mathbf{R}*} \gamma] \in \Gamma_A$, that is, \[ [f^{-1}_{\mathbf{R}*} \gamma]=[f^{-1}_{\mathbf{R}*} \gamma_{i_1} \cc \cdots \cc f^{-1}_{\mathbf{R}*} \gamma_{i_n}] =[\gamma_{j_1} \cdots \gamma_{j_s}]\] for some $A$-admissible cyclic word  $\gamma_{j_1} \cdots \gamma_{j_s}$. Since there is no cancelation between $\gamma_i$'s, if $f^{-1}_{\mathbf{R}*} \gamma_{i_j} \not\in \Gamma^+$ then the product of the last part of $f^{-1}_{\mathbf{R}*} \gamma_{i_j}$ and the first part of $f^{-1}_{\mathbf{R}*} \gamma_{i_{j+1}}$ should be equal to an element in $\Gamma$. Furthermore since the element $g$ only appears as the last letter for each $\gamma_i$, we have 
\[ [ f^{-1}_{\mathbf{R}*} \gamma_i] = [g_{i_{1,1}} \cdots g_{i_{1,n_1}} \cc g \cc g_{i_{2,1}} \cdots g_{i_{2, n_2}} \cc g \cc g_{i_{3,1}} \cdots g_{i_{j-1, n_{j-1}}} \cc g \cc g_{i_{j,1}} \cdots g_{i_{j, n_j}}]\]
where $g_{i_{j,k}} \ne g$ and  $g_{i_{j,k}} \in G \cup G^{-1}$ for all $i,j,k$ and the product $ g_{i_{j,1}} \cdots g_{i_{j, n_j}}  \cc g$ must be an element of $\Gamma$. 
It follows that  for each $\gamma_i \in \Gamma = \{ \gamma_1, \dots, \gamma_k\}$, we can  have $ [f^{-1}_{\mathbf{R}*} \gamma_i] = [\mu_i \cc \gamma_{i_1} \cc \cdots \gamma_{i_{n_i}} \cc \zeta_i]$ or $[ f^{-1}_{\mathbf{R}*} \gamma_i] = [\eta_i]$ where $\gamma_{i_1}, \dots, \gamma_{i_{n_i}} \in \Gamma$, and $ \zeta_i, \mu_i, \eta_i$ are words (possibly an identity element) in  $\pi_1(X(\mathbf{R}), P_{fix})$ with the following properties
\begin{itemize}
\item all three $\zeta_i, \eta_i, \mu_i$ are reduced,
\item the letter $g$ doesn't appear in $\zeta_i$ and $\eta_i$, 
\item the letter $g$ only appears as the last letter of $\mu_i$, and
\item $\zeta_i$ does not start with the letter $g^{-1}$.
\end{itemize}
Let us denote $I_1 \subset \{ 1, \dots, k\}$ a set of indices  such that
 \[ \text{if } \  i \in I_1,\quad \text{ then} \ \ f^{-1}_{\mathbf{R}*} \gamma_i = \mu_i \cc \gamma_{i_1} \cc \cdots \gamma_{i_{n_i}} \cc \zeta_i, \quad  \text{for some }\  \gamma_{i_1}, \dots \gamma_{i_n} \in \Gamma, \zeta_i, \mu_i \in  \pi_1(X(\mathbf{R}), P_{fix})\] 
 and use $I_2$ for the set of indices such that \[ \text{if } \quad i \in I_2,\quad \text{ then} \ \ f^{-1}_{\mathbf{R}*} \gamma_i =\eta_i, \qquad \text{for some } \qquad \eta_i \in \pi_1(X(\mathbf{R}), P_{fix}) \] 
If cyclically successive indices $i,j$ appear in some $A$-admissible words, to have $f^{-1}_{\mathbf{R}*}$-invariant $\Gamma_A$ one of the following situations should happen
\begin{itemize}\addtolength{\itemsep}{1ex}
\item If both $i, j \in I_1$, then the reduced word of $\zeta_i \cc \mu_j$ is an element of $\Gamma$.
\item If $i \in I_1$ and $j \in I_2$, then there are set of indices $ t_1, \dots, t_M$ such that successive indices $i, j, t_1, \dots, t_M$ appear in some $A$-admissible words, $t_1, \dots t_{M-1} \in I_2$, $t_M \in I_1$ and the reduced word of $\zeta_i \cc \eta_j \cc \eta_{t_1} \dots \eta_{t_{M-1}} \cc \mu_{t_M}$ is an element of $\Gamma$. 
\item If $i \in I_2$ and $j \in I_1$, then there are set of indices $ s_1, \dots, s_N$ such that  successive indices $ s_1, \dots, s_N,i,j$ appear in some $A$-admissible words, $s_1 \in I_1$, $s_2 \dots s_N \in I_2$ and the reduced word of $\zeta_{s_1} \cc \eta_{s_2} \dots \eta_{s_N} \cc \eta_{i } \cc \mu_j$ is an element of $\Gamma$. 
\item  If both  $i, j \in I_2$, then there are set of indices $ s_1, \dots, s_M$ and $ t_1, \dots, t_M$ such that successive indices $ s_1, \dots, s_N,i,j,t_1, \dots t_M$ appear in some $A$-admissible words, $s_1, t_M \in I_1$, $s_2, \dots, s_N, t_2 \dots t_M \in I_2$ and the reduced word of  $\zeta_{s_1} \cc \eta_{s_2} \dots \eta_{s_N} \cc \eta_{i }\cc \eta_j \cc \eta_{t_1} \dots \eta_{t_{M-1}} \cc \mu_{t_M}$ is an element of $\Gamma$. 
\end{itemize}


Recall that $\Gamma$ is a finite set of reduced words with respect to a set of generators $G$ with the property that there is $g \in G \cup C^{-1}$ such that every $\gamma_j$ ends with $g$ and starts with a letter not equal to $g, g^{-1}$. Let $\Delta$ be a finite set of reduced (non-cyclic) words in $\pi_1(X(\mathbf{R}), P_{fix})$ with respect to a set of generators $G$
\begin{equation*}
\begin{aligned}
& \Gamma = \{ \gamma_1, \dots, \gamma_k\}\\
& \Delta = \bigcup_{i \in I_1} \{ \zeta_i, \gamma_{i_1}, \dots \gamma_{i_{n_i}}, \mu_i\} \cup \bigcup_{i \in I_2} \{ \eta_i\} . \\
\end{aligned}
\end{equation*}
Let $V$ denote a linear span of $\Gamma$ and $W$ denote a linear span of $\Delta$. We define two linear maps $S,M: V \to W$ in the following way
\begin{itemize}
\item \textit{Splitting map} $S:V \to W$:
\begin{equation*}
S: \left\{ \begin{aligned}
&\gamma_i \mapsto \mu_i + \gamma_{i_1} + \cdots+ \gamma_{i_{n_i}} + \zeta_i, \qquad \text{if  } \ i \in I_1\\
&\gamma_i \mapsto \eta_i,\qquad \text{if  } \ i \in I_2\\ 
\end{aligned} \right.
\end{equation*}
\item \textit{Merging map} $M:V \to W$:
\begin{equation*}
M: \left\{ \begin{aligned}
&\gamma_i \mapsto \gamma_i, \qquad \text{if  }\ \gamma_i \in \Delta\\
&\gamma_i \mapsto \zeta_i + \eta_{i_1} + \cdots \eta_{i_s} + \mu_i, \ \ \text{if }\ \  \gamma_i \not\in \Delta, \ \text{and}\  \gamma_i = \zeta_i \cc \eta_{i_1} \cdots \eta_{i_s} \cc \mu_i\\
\end{aligned}\right.
\end{equation*}
\end{itemize}

\begin{lem}
Both a Splitting map, $S$ and a Merging map $M$ maps a positive span of $\Gamma$, $Sp^+ \Gamma \subset V$ to a positive span of $\Delta$, $Sp^+ \Delta \subset W$.
\end{lem}
\begin{proof}
For both $S$ and $M$, the image of $\gamma_i$ is given by positive sum of elements in $\Delta$. This lemma follows from the fact that the matrix representations for $S$ and $M$ are given by matrices with positive entries. 
\end{proof}

\begin{lem}\label{L:Grate}
If $\Gamma_A$ is $f^{-1}_{\mathbf{R}*}$-invariant, then for each $[\gamma] \in \Gamma_A$ we have 
\[ M \phi([\gamma])_\# = S [\gamma]_\# \]
\end{lem}

\begin{proof}
Let  $[\gamma] \in \Gamma_A$ with $\gamma = \gamma_{i_1} \cc \cdots \gamma_{i_n}$. Then $\phi[\gamma] = [f^{-1}_{\mathbf{R}*} \gamma] = [^{-1}_{\mathbf{R}*} \gamma_{i_1} \cdots f^{-1}_{\mathbf{R}*} \gamma_{i_n}] $
For each $j=1, \dots n$ we have $f^{-1}_{\mathbf{R}*} \gamma_{i_j}  = \prod_{\delta_{s_j} \in \Delta} \delta_{s_j}$, which determines $S \gamma_{i_j}$. On the other hand $\phi[\gamma]$ is determined after we combine $\zeta$'s, $\mu$'s and $\eta$'s. The merging map $M$ is decompose each $\gamma \in \Delta$ into sum of $\zeta$'s, $\mu$'s, and $\eta$'s. Thus by counting the number of each element in $\Delta$, we have  $M \phi([\gamma])_\# = S [\gamma]_\#$.
%$[\gamma]_\# =\sum  n_i(\gamma) \gamma_i$ where $n_i(\gamma)$ is the number of $\gamma_i$ in $\gamma$. Thus we have \[ S[\gamma]_\# = \sum n_i S \gamma_i .\]
\end{proof}
 
 Since the splitting map, $S$ and the merging map, $M$ are linear, it is easier to connect to the growth rate of $[\gamma]_\#$ under the iterations of $\phi$. 

\begin{thm}\label{T:Grate} Let $\Delta$ is a finite set of reduced words in $G$. Let $V = \text{Span}\, \Gamma$ be a linear span of $\Gamma$ and $W =  \text{Span}\,  \Delta$ be a linear span of $\Delta$. Suppose there are two one-to-one linear maps $T_i: V \to W$, $i=1,2$ such that both linear maps $T_i ( \text{Sp}^+ \Gamma) = \text{Sp}^+ \Delta$. Also suppose that  \[ T_2  \phi ([\gamma])_\# \ = T_1([\gamma]_\#),\qquad \text{for all  } \gamma \in \Gamma_A \]
where $\phi$ is the induced action $f^{-1}_{\mathbf{R}*}$ on $\pi_1(X(\mathbf{R}))$ and $[\gamma]_\# = \sum_i n_i(\gamma) \gamma_i$. 
If there is $v_\lambda \in \text{Sp}^+\Gamma$ such that $T_1 v_\lambda = \lambda \, T_2 v_\lambda$ for some $\lambda >1$, then the growth rate of the induced action on the fundamental group \[\rho(f^{-1}_{\mathbf{R}*}|_{\pi_1 (X(\mathbf{R}))}) \ge \lambda.\]
\end{thm}

\begin{proof}
Since the rank of $T_2 = \text{dim} V$, there is a left inverse $T_{2\, left}^{-1}$. And $v_\lambda$ is an eigenvector of $T_{2\, left}^{-1}T_1$ corresponding to an eigenvalue $\lambda>1$.  Because both $T_1$ and $T_2$ are one-to-one, for each $[\gamma] \in \Gamma_A$ and $n\ge 0$ there is $[\gamma' ] \in \Gamma_A$ such that \[ \phi([\gamma'] )_\# = (T_{2\, left}^{-1}T_1)^n [\gamma]_\#. \] 
Since $T_1 v_\lambda = \lambda \, T_2 v_\lambda$, for any left inverse $T_{2\, left}^{-1}$, $v_\lambda$ is an eigenvector associated with an eigenvalue $\lambda$ for $T_{2\, left}^{-1} T_1$. Since $v_\lambda$ is an eigenvector corresponding an eigenvalue $\lambda>1$, we have a sequence $[\gamma]_n \in \Gamma_A$ such that  \[ ([\gamma]_n) _\# = (T_{2\, left}^{-1}T_1)^n [\gamma]_\#  = c \lambda^n v_\lambda + v_n\]  for some positive constant $c$ and $v_n \in \text{Sp}^+ \Gamma \subset V$. 
It follows that \[\sup_{\gamma \in \Gamma_A} \left\{ \limsup_{n \to \infty} (\ell_\Gamma( \phi^n \gamma))^{1/n}  \right \} \ge \lambda \] and therefore \[\rho(f^{-1}_{\mathbf{R}*}|_{\pi_1 (X(\mathbf{R}))}) \ge \lambda.\]
\end{proof}

\begin{rem} In this paper, we are not claiming the existence of an invariant set of conjugacy classes of $A$-admissible words. For those cases we tried, we found the invariant set $\Gamma$ by iterating a generator for about $4 (n_1+n_2+n_3)$ times. For large $n_1+n_2+n_3$, it was computationally hard to iterate on our laptop computer. 

We also point out that we always get the same invariant set $\Gamma$ regardless of the choice of an initial word for iterations.
\end{rem}




